Numerically exact mimicking of quantum gas microscopy for interacting lattice fermions

A numerical method is presented for reproducing fermionic quantum gas microscope experiments in equilibrium. By employing nested componentwise direct sampling of fermion pseudo-density matrices, as they arise naturally in determinantal quantum Monte Carlo (QMC) simulations, a stream of pseudo-snapshots of occupation numbers on large systems can be produced. There is a sign problem even when the conventional determinantal QMC algorithm can be made sign-problem free, and every pseudo-snapshot comes with a sign and a reweighting factor. Nonetheless, this "sampling sign problem" turns out to be weak and manageable in a large, relevant parameter regime. The method allows to compute distribution functions of arbitrary quantities defined in occupation number space and, from a practical point of view, facilitates the computation of complicated conditional correlation functions. While the projective measurements in quantum gas microscope experiments achieve direct sampling of occupation number states from the density matrix, the presented numerical method requires a Markov chain as an intermediate step and thus achieves only indirect sampling, but the full distribution of pseudo-snapshots after (signed) reweighting is identical to the distribution of snapshots from projective measurements

==> suppmat-content.tex <==
%%%%%%%%%% Merge with supplemental materials %%%%%%%%%%
\pagebreak
\widetext
\begin{center}
\textbf{SUPPLEMENTAL MATERIAL} \\
\vspace{0.25cm}
\textbf{Numerically exact quantum gas microscopy for interacting lattice fermions} \\
\vspace{0.4cm}
Stephan Humeniuk$^{\text{1}}$, Yuan Wan$^{\text{1,2,3}}$ \\
\vspace{0.25cm}
$ \prescript{1}{}{\textit{Institute of Physics, Chinese Academy of Sciences, Beijing 100190, China}}$\\
$ \prescript{2}{}{\textit{University of Chinese Academy of Sciences, Beijing 100049, China}} $ \\
$ \prescript{3}{}{\textit{Songshan Lake Materials Laboratory, Dongguan, Guangdong 523808, China}} $

\end{center}
%%%%%%%%%% Merge with supplemental materials %%%%%%%%%%

%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{page}{1}
\setcounter{section}{0}
\makeatletter
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%

Here we provide a proof of a key equation in the main text, details for an efficient implementation of the algorithm,
a parameter scan of the sampling sign problem, and additional data on the polaron problem. 
The sections of the supplemental material are organized as follows. 
\begin{enumerate}
 \item Inductive proof of the expression for the marginals of the joint quasiprobabilities Eq.~\eqref{eq:joint_quasiprob_marginal} in the main text.
 \item Exploiting the block structure in Eq.~\eqref{eq:correction_term} of the main text.
 \item Parameter dependence of the sampling sign problem at and away from half filling.
 \item Code verification using exact diagonalization on a small system and by symmetry inspection of spin-only microstates around an 
 isolated hole on a large system. 
 \item Additional data for the polaron problem and comparison with the data of the quantum gas microscope experiment of Ref.~\cite{Koepsell2019}.
\end{enumerate}


% =====================================================================================
\section{Inductive proof of Eq.~(5) in the main text} 
\label{app:proof}
% =====================================================================================

Let 
\begin{equation}
G^{(0)}_{i_{\alpha}, j_{\beta}} = \langle \hat{c}_{i_{\alpha}} \hat{c}_{j_{\beta}}^{\dagger} \rangle_0 
\label{eq:def_G0}
\end{equation}
be the single-particle Green's function of a free fermion system, and $\alpha, \beta \in \{1,\ldots, D\}$. 
First we prove the well-known fact that 
Wick's theorem for higher-order correlation functions can be expressed in the compact determinant  form
\begin{equation}
 \left\langle \left(\hat{c}_{i_1} \hat{c}_{j_1}^{\dagger} \right)  \left(\hat{c}_{i_2} \hat{c}_{j_2}^{\dagger}\right) \cdots  \left(\hat{c}_{i_n} \hat{c}_{j_n}^{\dagger} \right) \right\rangle_0 
          = \det\left( G^{(0)}_{I=\{i_1, i_2, \ldots, i_n \}; J=\{j_1, j_2, \ldots, j_n \}}\right) \equiv \left[ G^{(0)} \right]_{I;J}.
 \label{eq:Wick_determinant}
\end{equation}
% % % \begin{equation}
% % % G^{(0)}_{i_{\alpha}, j_{\beta}} = \langle \hat{c}_{i_{\alpha}} \hat{c}_{j_{\beta}}^{\dagger} \rangle_0 
% % % \label{eq:def_G0}
% % % \end{equation}
We use the convention that $[A]_{I;J}$ refers to the determinant of the submatrix of $A$ whose row index (column index) runs in the set $I$ ($J$),
which is the ``inclusive'' definition of the minor. 

The proof goes by induction. The case $n=1$ is true by virtue of the definition \eqref{eq:def_G0}.
In the induction step, we use Wick's theorem, writing all non-vanishing contractions
for a product of $n+1$ pairs of fermionic operators as
\begin{align}
&\left\langle \left( \hat{c}_{i_1} \hat{c}_{j_1}^{\dagger} \right) \cdots \left( \hat{c}_{i_{n+1}} \hat{c}_{j_{n+1}}^{\dagger} \right) \right\rangle_0
 = - G^{(0)}_{i_1, j_{n+1}} \left\langle \left(\hat{c}_{i_{n+1}} \hat{c}_{j_1}^{\dagger} \right) \left( \hat{c}_{i_2} \hat{c}_{j_2}^{\dagger} \right) \cdots \left( \hat{c}_{i_n} \hat{c}_{j_n}^{\dagger} \right) \right \rangle_0 \nonumber \\
 &- \sum_{k=2}^{n-1} G^{(0)}_{i_k, j_{n+1}} \left \langle \left( \hat{c}_{i_1} \hat{c}_{j_1}^{\dagger} \right) \left( \hat{c}_{i_2} \hat{c}_{j_2}^{\dagger} \right)  \cdots 
                   \left( \hat{c}_{i_{n+1}} \hat{c}_{j_k}^{\dagger} \right) \left( \hat{c}_{i_{k+1}} \hat{c}_{j_{k+1}}^{\dagger} \right) \cdots 
                   \left( \hat{c}_{i_{n}} \hat{c}_{j_n}^{\dagger} \right)         \right \rangle_0  \nonumber \\
 &- G^{(0)}_{i_n, j_{n+1}} \left\langle \left( \hat{c}_{i_1} \hat{c}_{j_1}^{\dagger} \right) \cdots \left( \hat{c}_{i_{n-1}} \hat{c}_{j_{n-1}}^{\dagger} \right) \left( \hat{c}_{i_{n+1}} \hat{c}_{j_{n+1}}^{\dagger} \right)\right\rangle_0 \nonumber \\
 &+ G^{(0)}_{i_{n+1}, j_{n+1}} \left \langle \left( \hat{c}_{i_1} \hat{c}_{j_1}^{\dagger} \right) \cdots \left( \hat{c}_{i_n} \hat{c}_{j_n}^{\dagger} \right) \right \rangle_0.
 \label{eq:after_generalized_Wick}
\end{align}
The minus-sign, e.g. in the second line of Eq.~\eqref{eq:after_generalized_Wick}, 
comes from the permutation of $\hat{c}_{i_{n+1}}$ with $\hat{c}_{j_k}^{\dagger}$.
Using the induction hypothesis Eq.~\eqref{eq:Wick_determinant}, 
valid for $n$ pairs of fermionic operators,
the remaining correlators in Eq.~\eqref{eq:after_generalized_Wick}
can be expressed as determinants
\begin{align}
 \left\langle \left( \hat{c}_{i_1} \hat{c}_{j_1}^{\dagger} \right) \cdots \left( \hat{c}_{i_{n+1}} \hat{c}_{j_{n+1}}^{\dagger} \right) \right\rangle_0 = 
 &- G_{i_1, j_{n+1}}^{(0)} \cdot\det
   \begin{pmatrix}
    G_{i_{n+1}, j_1}^{(0)} & G_{i_{n+1},j_2}^{(0)} & \cdots & G_{i_{n+1},j_n}^{(0)} \\
    G_{i_2, j_1}^{(0)}     & G_{i_2,j_2}^{(0)}     & \cdots & G_{i_2,j_n}^{(0)}     \\
    \vdots                 & \vdots 		   & \ddots & \vdots 		    \\
    G_{i_n, j_1}^{(0)}     & G_{i_n,j_2}^{(0)}     & \cdots & G_{i_n,j_n}^{(0)}
   \end{pmatrix}  \nonumber \\
 &- G_{i_2, j_{n+1}}^{(0)} \cdot\det
   \begin{pmatrix}
    G_{i_1, j_1}^{(0)} & G_{i_1,j_2}^{(0)} & \cdots & G_{i_1,j_n}^{(0)} \\
    G_{i_{n+1}, j_1}^{(0)}     & G_{i_{n+1},j_2}^{(0)}     & \cdots & G_{i_{n+1},j_n}^{(0)}     \\
    \vdots                 & \vdots 		   & \ddots & \vdots 		    \\
    G_{i_n, j_1}^{(0)}     & G_{i_n,j_2}^{(0)}     & \cdots & G_{i_n,j_n}^{(0)}
   \end{pmatrix}
 - \cdots \nonumber \\
 &- G_{i_n, j_{n+1}}^{(0)} \cdot\det
   \begin{pmatrix}
    G_{i_1, j_1}^{(0)} & G_{i_1,j_2}^{(0)} & \cdots & G_{i_1,j_n}^{(0)} \\
        \vdots                 & \vdots 		   & \ddots & \vdots 		    \\
    G_{i_{n-1}, j_1}^{(0)}     & G_{i_{n-1},j_2}^{(0)}     & \cdots & G_{i_{n-1},j_n}^{(0)}     \\
    G_{i_{n+1}, j_1}^{(0)}     & G_{i_{n+1},j_2}^{(0)}     & \cdots & G_{i_{n+1},j_n}^{(0)}
   \end{pmatrix} \nonumber \\
 &+ G_{i_{n+1}, j_{n+1}}^{(0)} \cdot\det
   \begin{pmatrix}
    G_{i_1, j_1}^{(0)} & G_{i_1,j_2}^{(0)} & \cdots & G_{i_1,j_n}^{(0)} \\
    G_{i_2, j_1}^{(0)}     & G_{i_2,j_2}^{(0)}     & \cdots & G_{i_2,j_n}^{(0)} \\
	\vdots                 & \vdots 		   & \ddots & \vdots 		    \\
    G_{i_n, j_1}^{(0)}     & G_{i_n,j_2}^{(0)}     & \cdots & G_{i_n,j_n}^{(0)}
   \end{pmatrix}. \label{eq:induction_step} 
\end{align} 
By rearranging rows in \eqref{eq:induction_step}, it can be concluded that \eqref{eq:induction_step}
is the expansion of the $(n+1) \times (n+1)$ determinant 
\begin{equation}
 \det 
 \begin{pmatrix}
  G_{i_1,j_1}^{(0)} & G_{i_1,j_2}^{(0)} & \cdots & G_{i_1,j_{n+1}}^{(0)} \\
  G_{i_2,j_1}^{(0)} & G_{i_2,j_2}^{(0)} & \cdots & G_{i_2,j_{n+1}}^{(0)} \\
  \vdots            &   \vdots          & \ddots & \vdots          \\
  G_{i_{n+1},j_1}^{(0)}   & G_{i_{n+1},j_2}^{(0)}   & \cdots & G_{i_{n+1}, j_{n+1}}^{(0)}
 \end{pmatrix}
\end{equation}
along the last column according to Laplace's formula. This completes the inductive proof.
Except for the last determinant in Eq.~\eqref{eq:induction_step}, row exchanges are necessary to obtain the 
correct submatrix structure. 
In the determinant accompanying the single-particle Green's 
function $G_{i_k, j_{n+1}}^{(0)}$ in Eq.~\eqref{eq:induction_step}
we need to perform $(n-k)$ row exchanges which results in 
a factor $(-1)^{n-k}$ such that the total sign is $(-1)^{n-k+1}$,
which is identical to the alternating factor $(-1)^{n+1+k}$ coming from Laplace's formula.

Eq.~\eqref{eq:joint_quasiprob_marginal} differs from Eq.~\eqref{eq:Wick_determinant} in that instead of pairings $(\hat{c}_{i_k} \hat{c}_{j_k}^{\dagger})$  
there are projectors of the form
\begin{equation}
 \Pi_k = n_k \hat{c}_{j_k}^{\dagger} \hat{c}_{j_k} + (1 - n_k) \hat{c}_{j_k} \hat{c}_{j_k}^{\dagger}.
 \label{eq:projector_k}
\end{equation}
Depending on whether $n_k=0$ or $n_k=1$, only one of either terms in \eqref{eq:projector_k} applies. 
Let us replace for the moment only the $k$-th pairing $(\hat{c}_{i_k} \hat{c}_{j_k}^{\dagger})$ in Eq.~\eqref{eq:Wick_determinant} by $\Pi_k$. 
If $n_k = 0$, the resulting expression is covered by Eq.~\eqref{eq:Wick_determinant}. The case $n_k = 1$ is different since 
$\hat{c}_{j_k}^{\dagger}$ is to the right of $\hat{c}_{j_k}$. Using $\hat{c}_{j_k}^{\dagger} \hat{c}_{j_k} = 1 - \hat{c}_{j_k} \hat{c}_{j_k}^{\dagger}$, one obtains
\begin{equation}
\langle (\hat{c}_{i_1} \hat{c}_{j_1}^{\dagger} \cdots \Pi_k \cdots (\hat{c}_{i_n} \hat{c}_{j_n}^{\dagger}) \rangle_{0} 
= (-1)^{n_k}  n_k  \left[\det\left( G^{(0)}_{I \backslash j_k, J \backslash j_k} \right) - \det(G^{(0)}_{I,J}) \right]
\label{eq:commute_annihilator_creator}
\end{equation}
To make the connection with Eq.~\eqref{eq:joint_quasiprob_marginal} we consider the matrix 
\begin{equation}
 \left( \tilde{G}^{(0)} \right)_{ij} = \left( G^{(0)} \right)_{ij} - n_k \delta_{i,j_k} \delta_{j, j_k}
 \label{eq:Gtilde}
\end{equation}
and develop its determinant with respect to the $k$-th column:
\begin{align}
 \det(\tilde{G}) &= \sum_{l=1}^{n} (-1)^{l + k} \left( \tilde{G^{(0)}} \right)_{i_l, j_k}  \left[ \tilde{G^{(0)}} \right]_{I \backslash i_l, J\backslash j_k} \\
 &= \sum_{l=1}^{n} (-1)^{l+k} \left( G^{(0)} \right)_{i_l, j_k} \left[ G^{(0)} \right]_{I \backslash i_l, J \backslash j_k} - n_k (-1)^{2k} \left[ G^{(0)} \right]_{I \backslash j_k, J \backslash j_k} \label{eq:undo_Laplace}
\end{align}
Here, angular braces $( \cdot )$ denote matrix elements and square brackets $[ \cdot ]$ denote the inclusive definition of the minor. 
Note that the minors $\left[ \tilde{G^{(0)}} \right]_{I \backslash i_l, J \backslash j_k} = \left[ G^{(0)} \right]_{I\backslash i_l, J \backslash j_k}$ 
since $\tilde{G^{(0)}}$ and $G^{(0)}$ only differ in the element $(j_k, j_k)$ which is excluded from the minors.
Now, one can recognize in the first sum Eq.~\eqref{eq:undo_Laplace} the Laplace expansion of $G^{(0)}$ with respect to the $k$-th column and 
undo it again to recover $\det(G^{(0)})$:
\begin{equation}
 \det\left(\tilde{G^{(0)}}\right) = \det\left( G^{(0)} \right) - n_k \left[ G^{(0)} \right]_{I \backslash j_k, J \backslash j_k}.
 \label{eq:undo_Laplace_expansion}
\end{equation}
Eq.~\eqref{eq:undo_Laplace_expansion} is identical to Eq.~\eqref{eq:commute_annihilator_creator}, which proves that 
\begin{align}
\langle (\hat{c}_{i_1} \hat{c}_{j_1}^{\dagger}) \cdots \Pi_k \cdots (\hat{c}_{i_n} \hat{c}_{j_n}^{\dagger}) \rangle_{0} = \det 
\begin{pmatrix}
G^{(0)}_{i_1, j_1} & G^{(0)}_{i_1, j_2} & \cdots & \cdots & G^{(0)}_{i1, j_n} \\
G^{(0)}_{i_2, j_1} & G^{(0)}_{i_2, j_2} & \cdots & \cdots & G^{(0)}_{i2, j_n} \\
\vdots       & \vdots       & \ddots & \cdots &  \vdots     \\
\vdots       & \vdots       & G^{(0)}_{j_k, j_k} - n_k & \cdots &  \vdots       \\
\vdots       & \vdots       & \vdots 	         & \ddots &  \vdots       \\
G^{(0)}_{i_n, j_1} & G^{(0)}_{i_n, j_2} & \cdots & \cdots & G^{(0)}_{i_n, j_n} \\
\end{pmatrix}.
\label{eq:proof_one_projector}
\end{align}
Repeatedly replacing each pairing $(\hat{c}_{i_l} \hat{c}_{j_l}^{\dagger})$ in Eq.~\eqref{eq:Wick_determinant} by a projector 
$\Pi_l$ of the form \eqref{eq:projector_k} and repeating the derivation from \eqref{eq:Gtilde} to \eqref{eq:proof_one_projector}, 
with a Laplace expansion carried out with respect to the $l$-th column, completes the proof of Eq.~\eqref{eq:joint_quasiprob_marginal}.


\section{Exploitation of block matrix structure}
\label{app:block_determinant}

In the following, it is understood that $G \equiv G^{(0)}$ denotes a free-fermion Green's function,
and we drop the superscript.
Eq.~\eqref{eq:joint_quasiprob_marginal} implies that the expressions for the joint quasiprobability 
distributions of successive numbers of components 
are related by a block matrix structure. 
Using the formula for the determinant of a block matrix and noticing that $G(y,y)$ is just a number:
\begin{align}
 p(x_1, x_2, \ldots, x_{k-1}; y) &= \frac{1}{Z} \det 
 \left(
 \begin{array}{c|c}
 \raisebox{-35pt}{{\huge\mbox{{$X_{k-1}$}}}} & G(x_1, y) \\
                                       & G(x_2, y) \\
				       & \vdots    \\ 
				       & G(x_{k-1}, y) \\ \hline
 G(y,x_1) \, G(y,x_2) \, \cdots \, G(y,x_{k-1}) & G(y,y)  
 \end{array}
 \right)\\
 &= \frac{1}{Z} \det(X_{k-1}) \left[G(y,y) - \sum_{i,j=1}^{k-1} G(y,x_i) \left[ X_{k-1}^{-1}\right]_{i,j} G(x_j,y) \right].
\end{align}

Given that $X_{k-1}$ is itself a block matrix 
\begin{align}
 X_{k-1} &=
 \left(
 \begin{array}{c|c}
 \raisebox{-35pt}{{\huge\mbox{{$X_{k-2}$}}}} 			  & G(x_1, x_{k-1}) \\
								  & G(x_2, x_{k-1}) \\
								  & \vdots    \\ 
								  & G(x_{k-2}, x_{k-1}) \\ \hline
 G(x_{k-1},x_1) \, G(x_{k-1},x_2) \, \cdots \, G(x_{k-1},x_{k-2}) & G(x_{k-1},x_{k-1})  
 \end{array}
 \right)
\end{align} 
with $G(x_{k-1},x_{k-1})$ just a number and assuming that the inverse $X_{k-2}^{-1}$ is already known, one 
can make use of the formula for the inversion of a block matrix to compute the inverse of $X_{k-1}$ in 
an economical way.
We define
\begin{equation}
 g \equiv G(x_{k-1}, x_{k-1}) - \sum_{i,j=1}^{k-2} G(x_{k-1}, x_i) \left[ X_{k-2}^{-1} \right]_{i,j} G(x_j, x_{k-1}) 
\end{equation}
and recognize that
\begin{equation}
 g = \frac{p(x_1, x_2, \ldots, x_{k-1})}{p(x_1, x_2, \ldots, x_{k-2})} = p(x_{k-1}| x_{k-2}, \ldots, x_2, x_1),
\end{equation}
which means that we have computed $g$ already previously when sampling the $(k-1)$-th component.

Using the formula for the inverse of a block matrix
\begin{equation}
 X_{k-1}^{-1} = \left(
 \begin{array}{c|c}
   X_{k-2}^{-1} + g^{-1} \vec{u} \otimes \vec{v}^{T}    &    - g^{-1} \vec{u} \\  \hline
                - g^{-1} \vec{v}^{T}                    &      g^{-1}
 \end{array}
 \right),
\end{equation}
where 
\begin{align}
 [\vec{u}]_i &= \sum_{j=1}^{k-2} \left[ X_{k-2}^{-1} \right]_{ij} G(x_j, x_{k-1}), \\
 [\vec{v}^{T}]_j &= \sum_{i=1}^{k-2} \left[ X_{k-2}^{-1}\right]_{ij} G(x_{k-1}, x_i),
\end{align}
and 
\begin{equation}
 \left[\vec{u} \otimes \vec{v}^{T} \right]_{ij} = [\vec{u}]_{i} [\vec{v}^{T}]_{j}.
\end{equation}

Thus, the update $X_{k-2}^{-1} \rightarrow X_{k-1}^{-1}$ requires the computation of $\vec{u}$, $\vec{v}^{T}$,
and the exterior product $\vec{u} \otimes \vec{v}^{T}$, which is of order $\mathcal{O}((k-2)^2)$.
It is easy to see that the sampling of $N_p$ particle positions requires $\mathcal{O}(\sum_{i=1}^{N_p} i^2) = \mathcal{O}(N_p^3)$
floating point operations. It is not necessary to compute any inverse or determinant from scratch. 


% ========================================================================
\section{Sign problem for nested componentwise direct sampling at and away from half filling}
\label{app:sign_problem}
% ========================================================================

The severity of the conventional sign problem in the determinantal QMC algorithm is measured by the average sign
of the Monte Carlo weight 
\begin{equation}
\langle s \rangle = \frac{1}{N_{\text{HS samples}}} \sum_{\{ \vecbf{s}\}} \text{sign}(w_{\{ \vecbf{s} \}}^{\uparrow}  w_{\{ \vecbf{s} \}}^{\downarrow}),
\end{equation}
where the sum is over auxiliary field configurations of the Hubbard-Stratonovich samples.
\begin{figure}
% /home/stephan/Documents/FERMION_SNAPSHOTS/sign_problem_scan/DATA_av_sign/halffilling_Hubbard
\includegraphics[width=0.75\linewidth]{av_sign_vs_U.pdf}
\caption{Sampling sign problem at half filling. The probe area is the total $L \times L$ square system ($L=L_A$).
(a) Average sign of a pseudo-snapshot. (b) Average (unsigned) reweighting factor (full lines) and average maximum reweighting factor (dashed lines).
The red dashed-dotted line indicates a rough estimate of the threshold of maximum reweighting factors below which numerically exact results 
can be obtained with modest computational effort.}
\label{fig:av_sign_halffilling}
\end{figure}
\begin{figure}
\includegraphics[width=0.75\linewidth]{sign_problem_doped.pdf}
\caption{Conventional sign problem and sampling sign problem 
away from half filling: dependence on $U/t$. (a,c) Average sign ($\langle s \rangle$, full lines) and average sampling sign ($\langle \tilde{s} \rangle$, dashed lines);
(b,d) average reweighting factor (full lines) and average maximum reweighting factor (dotted lines).
The inverse temperature $\beta$ is in units of $1/t$.
The probe area is equal to the system size with $L_A=L=8$.}
\end{figure} 
\begin{figure}
 \includegraphics[width=0.75\linewidth]{sign_problem_temperature.pdf}
 \caption{Conventional sign problem  and sampling sign problem
 away from half filling: dependence on inverse temperature $\beta t$. System size $L_A=L=8$.}
\end{figure}
To quantify the ``sampling sign problem'' in the nested componentwise sampling algorithm we introduce 
the average sign of a snapshot, $\langle \tilde{s} \rangle$, which is given by
\begin{equation}
\langle \tilde{s} \rangle = \frac{1}{M}\sum_{\{ \vecbf{s}\}} \text{sign}(w_{\{ \vecbf{s} \}}^{\uparrow}  w_{\{ \vecbf{s} \}}^{\downarrow}) 
\sum_{i=1}^{N_{\text{snapshots per HS}}} \prod_{\sigma = \uparrow, \downarrow} \prod_{k=1}^{D} \text{sign}(p^{(i)}_{\{ \vecbf{s} \}}(n^{\sigma}_k)),
\end{equation}
where $M = N_{\text{HS samples}} \times N_{\text{snapshots per HS}}$ is the total number of generated snapshots.
Here, it is understood that snapshots drawn from the same HS sample, the number of which is $N_{\text{snapshots per HS}}$,
are multiplied by the sign of the 
corresponding Monte Carlo weight $w_{\{ \vecbf{s} \}}^{\uparrow}  w_{\{ \vecbf{s} \}}^{\downarrow}$,
in case that there is already a conventional sign problem at the level of the determinantal QMC algorithm. 
Note that within one HS sample, $\{ \vecbf{s} \}$, snapshots for spin-$\uparrow$ and spin-$\downarrow$
can be paired up arbitrarily into a full snapshot due to the statistical independence of the two spin species.

Furthermore, one can define the average (unsigned) reweighting factor 
\begin{equation}
R_{\text{av.}} = \frac{1}{M} \sum_{\{ \vecbf{s} \}} \sum_{i=1}^{N_{\text{snapshots per HS}}} 
\prod_{\sigma = \uparrow, \downarrow} \prod_{k=1}^{D} \mathcal{N}^{{\sigma}, (i)}_{k, \{ \vecbf{s}\}}
\end{equation}
and the average maximum reweighting factor, averaged over independent Markov chains, 
\begin{equation}
  R_{\text{av. max.}} = \frac{1}{N_{\text{Markov chains}}} \sum_{m=1}^{N_{\text{Markov chains}}} \max_{\substack{\text{snapshots } i \\ \text{from m-th Markov chain}}}\left( |R_i| \right).
\end{equation}
The average maximum reweighting $R_{\text{av. max.}}$ is the most relevant indicator of the severity of the sign problem
as it quantifies the ''inflation`` of value of an individual sample. Because the reweighting factor can fluctuate 
over several orders of magnitude, the average sign alone is not sufficient for a characterization of the ''sampling sign problem``. 

The snapshots generated in quantum gas microscope experiments originate from 
independent experimental runs whereas the pseudo-snapshots of the nested componentwise sampling 
are affected by the autocorrelation time inherent in the sampling of Hubbard-Stratonovich field 
configurations via the standard determinantal QMC algorithm. 
For large $U/t$, pseudo-snapshots taken from the same HS sample (and at the same imaginary time slice), differ mostly in the positions 
of holes and doubly occupied sites, while the spin background stays largely fixed. 

Additionally, pseudo-snapshots come with a sign and reweighting factor 
due to the non-Hermiticity of the pseudo-density operator within each HS sample. 
Therefore, experimental snapshots and pseudo-snapshots are not directly comparable. 
An important question is how many pseudo-snapshots $M$ are required to obtain a comparable precision 
of measurement quantities as from $M^{(\text{exp.})}$ experimental snapshots. 
Taking into account the average maximum reweighting factor, the effective number of pseudo-snapshots $M^{\prime}$
that is equivalent to $M^{(exp)}$ can be roughly estimated as 
\begin{equation}
 M^{\prime} = M / (\tau_{\text{AC}}^{\text{DQMC}} \times R_{\text{av.max.}}) \leftrightarrow  M^{(\text{exp.})}.
\end{equation}
Here, $\tau_{\text{AC}}^{\text{DQMC}} $ is some measure of the autocorrelation of the Markov chain generated 
by the standard determinantal QMC algorithm. 

The ''sampling sign`` deteriorates exponentially with the probe area $N_{\text{sites},A} = L_A^2$. Yet, an extent of the probe area $L_A \sim \xi(T/t, U/t, L)$,
where $\xi$ is the correlation length, is often sufficient for meaningful simulations. 

% ============================================================
\section{Code verification}
\label{app:benchmark_pentagon}
% ============================================================
For benchmarking purposes an irregular model instance of the Hubbard model on five sites (see inset in Fig.~\ref{fig:benchmark_5sites}(b)) is chosen
\begin{equation}
 \mathcal{H} = -\sum_{\langle i,j, \rangle, \sigma=\uparrow, \downarrow} t^{\sigma}_{ij}\left( c_{i,\sigma}^{\dagger} c_{j,\sigma} + h.c. \right) 
 + U \sum_{i=1}^{5} n_{i,\uparrow} n_{i,\downarrow}  - \sum_{\sigma = \uparrow, \downarrow}\mu_{\sigma} \sum_{i=1}^{5} n_{i,\sigma},
\end{equation}
which breaks translational, point group and spin rotational 
symmetry. The hopping matrix is identical for both spin species and reads
\begin{equation}
 [t^{\sigma}]_{i,j} = t
\begin{pmatrix}
0 & 0.7 & 1.1 & 0 & 0.8 \\
0.7 & 0 & 1.05 & 0.9 & 1.2 \\
1.1 & 1.05 & 0 & 1.0 & 0 \\
0 & 0.9 & 1.0 & 0 & 0 \\
0.8 & 1.2 & 0 & 0 & 0 \\
\end{pmatrix}
\label{eq:benchmark_hopping}
\end{equation}.
The onsite repulsion is $U/t=4$ and the chemical potential for spin up and down is 
$\mu_{\uparrow}/t=1.5$ and $\mu_{\downarrow}/t=1.8$, respectively; the inverse temperature is 
$\beta t = 4$ discretized into $N_{\tau} = 256$ Trotter time slices with $\Delta \tau t = \beta t / N_{\tau} = 1/64$.
Fig.~\ref{fig:benchmark_5sites} compares the probabilities $P(s)$ of all microstates $s$ in the occupation number basis 
with results from exact diagonalization. An enlarged view of Fig.~\ref{fig:benchmark_5sites}(a) is shown in Fig.~\ref{fig:benchmark_5sites}(b).
The occupation number state $\vec{n} = [n_{1, \uparrow} \ldots n_{5, \uparrow}; n_{1, \downarrow} \ldots n_{5, \downarrow}]$ with $n_{i,\sigma} \equiv n_{\alpha} \in \{0, 1\}$
is interpreted as a bitstring and is represented by the integer $s = \sum_{\alpha = 0}^{2 N_{\text{sites}}-1} n_{\alpha} 2^{\alpha}$.
With the knowledge of the eigenenergies $E_i$ and eigenvectors $|\phi_i \rangle$ of the Hamiltonian $\mathcal{H}$ the probability of 
an occupation number state $s$ is
\begin{equation}
 P(s) = \sum_{i=1}^{\text{dim}(H)} e^{-\beta E_i} |\langle s | \varphi_i \rangle |^2.
\end{equation}

\begin{figure}[h!]
\includegraphics[width=0.65\linewidth]{benchmark_pentagon.pdf}
\caption{Probabilities $P(s)$ of all microstates $s$ in the occupation number basis.
Comparison with exact diagonalization (ED) for the parameters shown in the upper panel and for the hopping matrix of Eq.~\eqref{eq:benchmark_hopping}. 
The total number of Fock samples is $10^7$, generated 
by 56 independent Markov chains.}
\label{fig:benchmark_5sites}
\end{figure} 
In order to demonstrate that the nested componentwise direct sampling method yields consistent microscopic states also for much larger system sizes, 
Fig.~\ref{fig:hole_spingb_environment} shows the probabilities of spin-only states on the eight sites around an isolated, mobile hole
for a system of $10 \times 10$ lattice sites at small doping. Only isolated holes, i.e. those surrounded exclusively by singly occupied sites, are considered 
(see Eq.~\eqref{eq:spinonly_env_projector} of the main text).
With the labelling of sites around a hole as shown in the right panel of Fig.~\ref{fig:hole_spingb_environment}, the spin environment is characterized 
by the state $\vec{\sigma} = [\sigma_{0} \sigma_{1} \ldots \sigma_{7}]$ where $\sigma_{p}=1$ 
if there is a spin-$\uparrow$ at position $p$ around the hole and $\sigma_{p}=0$ if it is a spin-$\downarrow$. 
With this convention, the state index in Fig.~\ref{fig:hole_spingb_environment} is given as $s = \sum_{p = 0}^{7} \sigma_{p} 2^{p}$. 
Fig.~\ref{fig:hole_spingb_environment} shows that there is a hierarchy of groups of states (right panel of Fig.~\ref{fig:hole_spingb_environment}).
Furthermore, states related by symmetry appear with approximately the same probability, 
which is not a built-in feature of the nested componentwise sampling algorithm and thus 
provides strong evidence that all relevant occupation number states are sampled with their correct probabilities. 

\begin{figure}[h!]
\includegraphics[width=1.0\linewidth]{hist_U12_L8_mu-2p0_beta2p5_all.pdf}
\caption{(a) Probabilities of spin-only states around an empty site as obtained from reweighted pseudo-snapshots
in the reference frame of the hole. Parameters: $U/t=12, \mu/t = -2, \beta t = 2.5$, $L \times L$
square lattice with $L=8$. 
For this system size, the average number of holes and doubles $\langle N_h \rangle \approx 1.50$ and $\langle N_d \rangle \approx 1.31$
so that the average number of excess holes is $\langle N_h \rangle - \langle N_d \rangle \approx 0.19$. 
With 56 independent Markov chains a total number of $70 \times 10^6$ occupation number samples of 
the entire system was obtained. 
In the reference frame of the hole, those states around the hole position are filtered out
which do not contain charge fluctuations (``spin-only states''). 
Per Hubbard-Stratonovich configuration, 200 direct sampling steps were performed during the Monte Carlo sweeps 
at different imaginary time slices. Trotter discretization $\Delta \tau t= 0.02$.
(b) Illustration of the most important spin-only states around an isolated hole which are marked in panel (a).
Dashed lines delineate different antiferromagnetic domains. }
\label{fig:hole_spingb_environment}
\end{figure}


\section{FCS of number of doublons and holes}
\label{app:FCS_doublons_holes}

Fig.~\ref{fig:FCS_doublons_holes} displays the doping dependence of the FCS of the number of doubly occupied sites 
$N_{d} = \sum_{i=1}^{N_{\text{sites}, A}} n_{i,\uparrow} n_{i,\downarrow}$  
and holes $N_h = \sum_{i=1}^{N_{\text{sites}, A}} \left(1 - n_{i,\uparrow} \right) \left(1 - n_{i,\downarrow} \right)$
for $U/t=12, \beta t = 4$ on an $L \times L$ system with $L=L_A=8$. 
\begin{figure}
% \includegraphics[width=0.95\linewidth]{FCS_Ndoublons_Nholes_L8_U12_beta4_doped.pdf}
\includegraphics[width=0.5\linewidth]{FCS_Ndoublons_Nholes_L8_U12_beta4_doped_2x1.pdf}
% /home/stephan/Documents/FERMION_SNAPSHOTS/full_counting/FCS_DATA/direct_sampling/doped_Hubbard/plots
\caption{FCS of the total number of doubly occupied sites $\langle N_d \rangle$ and holes $\langle N_h \rangle$, obtained from reweighted pseudo-snapshots
for different levels of hole doping (top and bottom panel). Dashed and dotted lines are binomial distributions (see main text).
Parameters: $U/t=12$, $\beta t = 4, L=8$.} 
\label{fig:FCS_doublons_holes}
\end{figure}
For small doping values, the FCS are well described by 
binomial distributions (dashed and dotted lines) which are generated by populating 
lattice sites independently with doublons (holes) with probability $p_d = \langle n_{\uparrow} n_{\downarrow} \rangle$ 
($p_h = \langle (1 - n_{\uparrow}) (1 - n_{\downarrow} \rangle) \rangle$).
according to the distribution 
$\mathcal{B}_{n,p}(x) = \begin{pmatrix} n \\ x\end{pmatrix} p^{x} (1-p)^{n-x}$ with $n=N_{\text{sites},A}$ and \mbox{$p \in \{p_d, p_h \}$}. 
In the strongly doped case (lower panel), the distribution of the number of holes can be modelled accurately 
by a ``shifted binomial'' distribution (dashed-dotted line), which 
is obtained by populating the lattice with holes arising from doublon-hole fluctuations according to a binomial distribution 
with parameter $p=p_d$ (since the number of doublon-hole pairs is approximately equal to the number of doublons) 
which is then shifted so that the distribution is centered about its mean.
Of course, for a large probe area and away from a critical point, the distribution of holes (doublons) should 
approach a Gaussian distribution which could be characterized 
by computing the mean and variance directly.
% % % Calculating the FCS of holes is useful for assessing whether an experimentally determined
% % % hole number distribution is intrinsic to the studied model 
% % % or corrupted, e.g. by atomic loss effects \cite{Koepsell2019}.


\section{Additional data for the polaron problem}
\label{app:additional_data}

\begin{figure}[b!]
% /home/stephan/Documents/FERMION_SNAPSHOTS/draft/no_polaron.svg
\includegraphics[width=0.95\textwidth]{no_polaron.pdf}
\caption{The three-point spin-charge correlation function $C_{|\vecbf{d}|=2}(|\vecbf{r}|)$ of Eq.~\eqref{eq:third_order_corr} 
computed on a $4 \times 4$ system (a-c) as well as a $6 \times 6$ 
system (d-g) with periodic boundary conditions and with parameters $U/t=14, \beta t = 2.5, \mu=-4.0, -4.5, \ldots, -6.5$.
The experimental data of Ref.~\cite{Koepsell2019}
are also shown for comparison. There, the system size is approximately $4 \times 6$ to $6 \times 6$ lattice sites (slightly inhomogeneous with open boundary conditions), interactions $U/t \approx 14$
and stated temperature $T = 1.4 J$, which corresponds to $T/t \approx 0.4$ (i.e. $\beta t = 2.5$) for $J= 4 t^2 / U$. 
In the quantum gas microscope experiment, there are on average $1.95(1)$ dopants present 
in each experimental realization (doublon-doped instead of hole-doped) \cite{Koepsell2019}. 
For our setting on a $4 \times 4$ system at $\mu/t=-4.0$, on the other hand, the average number of holes (hole-doped) 
is $\langle N_h \rangle = 0.72$, which is small enough for measuring the spin-environment of an \emph{isolated} dopant.
(d) Randomly chosen snapshots for $\mu/t=-4$ (left) and $\mu/t=-5$ (right).}
\label{fig:no_polaron}
\end{figure}
\begin{figure}
\includegraphics[width=0.5\textwidth]{FCS_Ndh_U14_L10_mu-3p0_beta2p5.pdf}
\caption{FCS of the number of doubly occupied ($N_d$) and empty sites ($N_h$) for the same parameters 
as in Fig.~\ref{fig:three_point_spincharge_corr} of the main text, which are $L=10, U/t=14, \mu/t = -3.0, \beta t = 2.5$. }
\label{fig:FCS_same_params_as_maintext}
\end{figure}
This section illustrates the significance of numerical simulations for exploring the parameter space. 
In agreement with Ref.~\cite{Blomquist2019AbInitio} for the $t-J$ model and the results of Fig.~\ref{fig:three_point_spincharge_corr} for the Hubbard model,
one can identify the joint condition $C_{|\vecbf{d}|=2}(|\vecbf{r}|=0) < 0$ and $C_{|\vecbf{d}|=2}(|\vecbf{r}|=1) > 0$ as a characteristic correlation pattern of a magnetic polaron. 
However, $C_{|\vecbf{d}|=2}(|\vecbf{r}|=0) < 0$ by itself occurs also for larger doping values where the antiferromagnetic spin background is too diluted to host polarons. 
Fig.~\ref{fig:no_polaron} juxtaposes the evolution of the three-point correlation function in the reference frame of a hole
\begin{equation}
C_{|\vecbf{d}|=2}(|\vecbf{r}|) = \frac{\langle n_{\vecbf{r}_0}^{(h)} S^{z}_{\vecbf{r}_0 + \vecbf{r} + \frac{\vecbf{d}}{2}} S^{z}_{\vecbf{r}_0 + \vecbf{r} - \frac{\vecbf{d}}{2}}\rangle }{ \langle n_{\vecbf{r}_0}^{(h)} \rangle}. 
\end{equation}
as a function of chemical potential $\mu/t$
for $L=4$ (c) and $L=6$ (e), respectively, with the distribution of the number of holes (b,g) and doubly occupied sites (a,f). 
Unlike in Eq.~\eqref{eq:third_order_corr} of the main text, for the study of the hole environment in Fig.~\ref{fig:no_polaron} 
no projection operator restricting the sites around the hole to be singly occupied has been applied 
prior to evaluating the correlation function.
The data points connected by a thick red line are taken from Fig.~4(c) of Ref.~\cite{Koepsell2019}.
From $\mu/t=-4$ to $\mu/t = -5.5$ the correlator $C_{|\vecbf{d}|=2}(|\vecbf{r}|)$ changes markedly
which leads to the conclusion that Fig.~4 of Ref.~\cite{Koepsell2019} is consistent 
with the disappearance rather than the presence of magnetic polarons, which is due to the relatively high level of doping chosen in Ref.~\cite{Koepsell2019}.
This picture is supported by visually comparing the two randomly selected pseudo-snapshots for $\mu/t=-4$ versus $\mu/t=-5$ in
Fig.~\ref{fig:no_polaron}(d). However, note that the pseudo-snapshots should not be taken at face value
since they come with a sign and a reweighting factor.
Fig.~S8
% % % ~\ref{fig:FCS_same_params_as_maintext} 
shows the FCS of the number of doubly occupied sites and holes for the same parameters 
as in Fig.~\ref{fig:three_point_spincharge_corr} of the main text, indicating that only a small number of excess holes is present
in the pseudo-snapshots. 

